Conditional Value-at-Risk for Reachability and Mean Payoff in Markov Decision Processes

We present the conditional value-at-risk (CVaR) in the context of Markov chains and Markov decision processes with reachability and mean-payoff objectives. CVaR quantifies risk by means of the expectation of the worst p-quantile. As such it can be used to design risk-averse systems. We consider not only CVaR constraints, but also introduce their conjunction with expectation constraints and quantile constraints (value-at-risk, VaR). We derive lower and upper bounds on the computational complexity of the respective decision problems and characterize the structure of the strategies in terms of memory and randomization.

==> macros.tex <==
% == LATEX
%\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

%\newcolumntype{L}{X}
%\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
%\newcolumntype{C}{>{\centering\arraybackslash}X}

% == SPACE

%\renewcommand{\baselinestretch}{0.975} % >=0.97

%\newcommand{\spacefu}{\vspace*{-1.2em}}
%\newcommand{\spacefl}{\vspace*{-0.8em}}
%\newcommand{\myspace}{\vspace*{-0.5em}}

% == SYMBOLS

\RequirePackage{marvosym}
\providecommand{\contradiction}{\Lightning}

% == BASIC OPERATORS

\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\pospart}{\lgroup}{\rgroup^+}
\DeclarePairedDelimiter{\negpart}{\lgroup}{\rgroup^-}
\DeclarePairedDelimiterX{\inner}[2]{\lange}{\rangle}{#1, #2}
\DeclarePairedDelimiter{\cardinality}{\lvert}{\rvert}
\DeclarePairedDelimiter{\set}{\lbrace}{\rbrace}
\DeclarePairedDelimiter{\tuple}{(}{)}
\DeclarePairedDelimiter{\listt}{[}{]}


% == SETS OPERATORS

\newcommand{\setcomplement}[1]{{#1}^c}
\newcommand{\powerset}[1]{\mathcal{P}(#1)}

\newcommand{\unionSym}{\cup}
\newcommand{\unionBin}{\mathbin{\unionSym}}
\newcommand{\strictunionSym}{\dot{\unionSym}}
\newcommand{\strictunionBin}{\mathbin{\dot{\unionSym}}}
\newcommand{\intersectionSym}{\cap}
\newcommand{\intersectionBin}{\mathbin{\intersectionSym}}
\newcommand{\UnionSym}{\bigcup}
\newcommand{\UnionBin}{\mathbin{\UnionSym}}
\newcommand{\strictUnionSym}{\dot{\UnionSym}}
\newcommand{\strictUnionBin}{\mathbin{\strictUnionSym}}
\newcommand{\IntersectionSym}{\bigcap}
\newcommand{\IntersectionBin}{\mathbin{\IntersectionSym}}

\newcommand{\union}{\unionBin}
\newcommand{\strictunion}{\strictunionBin}
\newcommand{\intersection}{\intersectionBin}
\newcommand{\Union}{\UnionSym}
\newcommand{\strictUnion}{\strictUnionSym}
\newcommand{\Intersection}{\IntersectionSym}


% == BASIC SETS

\newcommand{\Naturals}{\mathbb{N}}
\newcommand{\Rationals}{\mathbb{Q}}
\newcommand{\Reals}{\mathbb{R}}


% == OPERATORS

\newcommand{\gradient}{\nabla}
\newcommand{\laplacian}{\Delta}
\newcommand{\diff}{\partial}
\newcommand{\boundary}{\partial}
\DeclareMathOperator{\divergence}{div}
\DeclareMathOperator{\distance}{dist}
\DeclareMathOperator{\esssup}{ess sup}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\capacity}{cap}
\DeclareMathOperator{\signum}{signum}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\const}{const}
\DeclareMathOperator{\loc}{loc}
\DeclareMathOperator*{\argmax}{arg\, max}

\newcommand{\qee}{\hfill$\triangle$} % quod erat exemplandum

% == LOGIC

\newcommand{\boolor}{\vee}
\newcommand{\booland}{\wedge}
\newcommand{\boolOr}{\bigvee}
\newcommand{\boolAnd}{\bigwedge}
\newcommand{\boolnot}{\lnot}

\DeclareMathOperator{\ExistsOp}{\exists}
\DeclareMathOperator{\ForallOp}{\forall}

\newcommand{\LTL}{\operatorname{LTL}}
\newcommand{\CTL}{\operatorname{CTL}}
\newcommand{\PCTL}{\operatorname{pCTL}}
\newcommand{\Next}{\varbigcirc}
\newcommand{\LtlEventually}{\diamondsuit}
\newcommand{\LtlAlways}{\Box}
\newcommand{\LtlUntil}{\, \mathcal{U}}
\newcommand{\LtlWrelease}{\mathcal{W}}
\newcommand{\LtlLanguage}[1]{\mathcal{L}(#1)}
\newcommand{\true}{\texttt{tt}}
\newcommand{\false}{\texttt{ff}}


% == COMPLEXITY

\newcommand{\NP}{\mathbf{NP}}
\newcommand{\NEXP}{\mathbf{NEXP}}
\newcommand{\PSPACE}{\mathbf{PSPACE}}


% == PROBABILITY

\newcommand{\ProbSpace}{\Omega}
\newcommand{\event}{\omega}
\newcommand{\Salgebra}{\mathcal{F}}
\newcommand{\measure}{\mu}
\newcommand{\Probability}{\mathbb{P}}
\newcommand{\Expectation}{\mathbb{E}}
\newcommand{\Distributions}{\mathcal{D}}
\newcommand{\Borel}{\mathfrak{B}}


% == MC, MPD, Games

\newcommand{\States}{S}
\newcommand{\initstate}{s_0}

\newcommand{\MC}{\mathsf{M}}
\newcommand{\trans}{\delta}
\newcommand{\SCCs}{\mathsf{SCC}}
\newcommand{\BSCCs}{\mathsf{BSCC}}

\newcommand{\MDP}{\mathcal{M}}
\newcommand{\Trans}{\Delta}
\newcommand{\Actions}{\mathsf{A}}
\newcommand{\AvAct}{\mathsf{Av}}
\newcommand{\act}[1]{\AvAct(#1)}
\newcommand{\MECs}{\mathsf{MEC}}

\newcommand{\reachSet}{T}
\newcommand{\reward}{\mathbf{r}}

\newcommand{\run}{\rho}
\newcommand{\Runs}{\varOmega}
\newcommand{\finitePath}{\varrho}
\newcommand{\strategy}{\sigma}
\newcommand{\Strategies}{\Pi}

\newcommand{\Cone}{\mathsf{Cone}}
\newcommand{\Memory}{\mathsf{M}}

\newcommand{\ObjFun}{R}
\newcommand{\MP}{\ObjFun^\QueryObjMean}

\newcommand{\Prob}{\mathbb{P}}

\newtheorem{remark}{Remark}

\DeclareMathOperator{\CVaR}{CVaR}
\DeclareMathOperator{\VaR}{VaR}
\DeclareMathOperator{\Inf}{Inf}

\newcommand{\QEE}{\hfill$\triangle$} % quod erat exemplandum

\newcommand{\QueryMDP}{\mathsf{MDP}}
\newcommand{\QueryMC}{\mathsf{MC}}

\newcommand{\QueryCrit}{\mathbf{crit}}
\newcommand{\QueryObj}{\mathbf{obj}}
\newcommand{\QueryDim}{\mathbf{dim}}

\newcommand{\QueryCritExp}{\Expectation}
\newcommand{\QueryCritCVaR}{\CVaR}
\newcommand{\QueryCritVaR}{\VaR}

\newcommand{\QueryObjReach}{\mathsf{r}}
\newcommand{\QueryObjMean}{\mathsf{m}}
\newcommand{\QueryDimSingle}{\mathsf{single}}
\newcommand{\QueryDimMulti}{\mathsf{multi}}

\newcommand{\QueryThreshExp}{\mathsf{e}}
\newcommand{\QueryThreshCVaR}{\mathsf{c}}
\newcommand{\QueryThreshVaR}{\mathsf{v}}
\newcommand{\QueryProbCVaR}{\mathsf{p}}
\newcommand{\QueryProbVaR}{\mathsf{q}}

\newcommand{\QueryThreshExpVec}{\mathsf{\mathbf{e}}}
\newcommand{\QueryThreshCVaRVec}{\mathsf{\mathbf{c}}}
\newcommand{\QueryThreshVaRVec}{\mathsf{\mathbf{v}}}
\newcommand{\QueryProbCVaRVec}{\mathsf{\mathbf{p}}}
\newcommand{\QueryProbVaRVec}{\mathsf{\mathbf{q}}}

\newcommand{\QueryVec}[1]{\mathbf{#1}}

% OLD

%-- others

\newcommand{\vecl}[1]{\vec{#1}}
\newcommand{\val}{\vec{v}}
\newcommand{\dist}{\mathit{Dist}}
\newcommand{\poly}{\mathit{poly}}
\newcommand{\ub}{\textbf{U:\ }}
\newcommand{\lb}{\textbf{L:\ }}
\newcommand{\ubl}{\textbf{U}=\textbf{L:} }


\renewcommand{\Pr}[2]{\Prob^{#1}\hspace{-0.16em}\left[{#2}\right]}   %\Pr{strat}{state}{event}
%\newcommand{\PrS}[3]{\Prob^{#1}_{#2}\hspace{-0.16em}\left[{#3}\right]}   %\Pr{strat}{state}{event}
\newcommand{\expected}{\mathbb E}
\newcommand{\Ex}[2]{\expected^{#1}\hspace{-0.16em}\left[{#2}\right]}   %\Ex{strat}{state}{f}
%\newcommand{\ExS}[3]{\expected^{#1}_{#2}\hspace{-0.16em}\left[{#3}\right]}   %\Ex{strat}{state}{f}
%
%\newcommand{\ex}{\vecl{exp}}
%\newcommand{\sat}{\vecl{sat}}
%\newcommand{\satscalar}{\mathit{sat}}
%\newcommand{\psat}{\vecl{pr}}%{\vec{p^{sat}}}
%\newcommand{\psatscalar}{\mathit{pr}}%{\mathit{p^{sat}}}
%
%\newcommand{\lrLim}[1]{\mathrm{lr}(#1)}  %\lr{rew}{run}
%\newcommand{\lrSf}[1]{\mathrm{lr}_{\mathrm{sup}}(#1)}  %\lrS{rew}{run}
%\newcommand{\lrIf}[1]{\mathrm{lr}_{\mathrm{inf}}(#1)}  %\lrI{rew}{run}
%\newcommand{\lrInf}{\mathrm{lr}^{\mathrm{inf}}}  %\lrI{rew}{run}
%
%
%
%\newcommand{\pagewidth}{\textwidth}
%
%\newcounter{mycounter}
%\newcommand{\thmhelperpre}[2]{\newcommand{\theoremlike}[1]{\par\medskip\penalty-250\refstepcounter{theorem}{\bfseries\noindent##1 \ref{#1}.}\itshape}\theoremlike{#2}}
%\newcommand{\thmhelperpost}{\par\medskip%
%	\renewcommand{\theoremlike}[1]{\par\medskip\penalty-250\refstepcounter{theorem}{\bfseries\noindent##1 \thesection .\thetheorem.}\itshape}%
%}
%\newenvironment{refclaim}[1]{\thmhelperpre{#1}{Claim}}{\thmhelperpost}
%\newenvironment{refcorollary}[1]{\thmhelperpre{#1}{Corollary}}{\thmhelperpost}
%\newenvironment{reftheorem}[1]{\thmhelperpre{#1}{Theorem}}{\thmhelperpost}

%%%%%%%% Local and misc.:

\newcommand{\kd}[1]{\mathbbm{1}_{#1}} %Kronecker's delta for a
\newcommand{\kda}{\kd{a}} %Kronecker's delta for a
\newcommand{\reach}{\Diamond}%{\mathit{Reach}}
\newcommand{\stabi}[1]{\kappa_{#1}}
\newcommand{\lfa}{\mathit{lf}_a}
\newcommand{\vfreq}{\mathrm{Freq}}
\newcommand{\freq}{\mathrm{freq}}
\newcommand{\toss}{\mathit{toss}}
\newcommand{\leave}{\mathit{leave}}




